Coherent control and suppressed nuclear feedback of a single quantum dot hole qubit

Future communication and computation technologies that exploit quantum information require robust and well-isolated qubits. Electron spins in III-V semiconductor quantum dots, while promising candidates, see their dynamics limited by undesirable hysteresis and decohering effects of the nuclear spin bath. Replacing electrons with holes should suppress the hyperfine interaction and consequently eliminate strong nuclear effects. Using picosecond optical pulses, we demonstrate coherent control of a single hole qubit and examine both free-induction and spin-echo decay. In moving from electrons to holes, we observe significantly reduced hyperfine interactions, evidenced by the reemergence of hysteresis-free dynamics, while obtaining similar coherence times, limited by non-nuclear mechanisms. These results demonstrate the potential of optically controlled, quantum dot hole qubits.

==> Holedefs.tex <==
% Definitions to be used in "Complete control . . ."

% standard packages
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{graphicx}
\RequirePackage{color}
\RequirePackage[active]{srcltx}

%% unique to this
\newcommand\deltae{\ts\delta{e}}
\newcommand\deltah{\ts\delta{h}}
\newcommand{\prp}{p}
\newcommand{\te}{\ts\tau{eff}}

%%% Standard TL commands

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Long comments
\long\def\comment#1{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% To save typing on all math commands
\newcommand{\mathcommand}[3][0]{\newcommand{#2}[#1]{\ensuremath{#3}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Text subscripting
\newcommand{\ts}[2]{{#1}_{\textnormal{#2}}} %A math symbol with a text subscript
\newcommand{\tsc}[2]{{#1}_{\textsc{#2}}} %A math symbol with a text subscript, small caps

\newcommand{\partialby}[1]{\frac{\partial}{\partial{#1}}}
\newcommand{\sqpartialby}[1]{\frac{\partial^2}{\partial{#1}^2}}
\newcommand{\dbyd}[1]{\frac{d}{d#1}}
\mathcommand{\radtwo}{\sqrt{2}}
\mathcommand[1]{\oneover}{\frac{1}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Equation Environments
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\refeq}[1]{Eq.~\eqref{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% State labels
\mathcommand{\eup}{\uparrow}
\mathcommand{\edown}{\downarrow}
\mathcommand{\tup}{\uparrow\downarrow,\Uparrow}
\mathcommand{\tdown}{\uparrow\downarrow,\Downarrow}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Hamiltonian Notation
\newcommand{\ham}[1][]{\ensuremath{{H}_{\text{#1}}}} % symbol for hamiltonian (second quantized)
\newcommand{\hamdens}[1][]{\ensuremath{\mathcal{H}_{\text{#1}}}} %symbol for hamiltonian density
\newcommand{\tildehamdens}[1][]{\ensuremath{\tilde{\mathcal{H}}_{\text{#1}}}} %symbol for hamiltonian density with tilde
\newcommand{\barhamdens}[1][]{\ensuremath{\ts{\bar{\mathcal{H}}}{#1}}}
\mathcommand[1]{\supop}{\hat{#1}} % to promote an operator to a superoperator
\newcommand{\supham}[1][]{\ensuremath{\supop{H}_{\text{#1}}}} %symbol for hamiltonian superoperator
\mathcommand[1]{\hilbert}{\mathfrak{H}_{\text{#1}}} %symbol for Hilbert space
\newcommand{\aveham}[2][]{\bar{\mathcal{H}}^{(#2)}_{\text{#1}}} % Used for average Hamiltonian terms in paper
\mathcommand[2]{\avehamt}{\ts{\tilde{\mathcal{H}}}{#1}^{(#2)}} % Used for average Hamiltonian terms in paper

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Bra Ket notation
\mathcommand[1]{\smallket}{|#1\rangle}
\mathcommand[1]{\smallbra}{\langle #1|}
\mathcommand[1]{\bigket}{\bigl|#1\bigr\rangle}
\mathcommand[1]{\bigbra}{\bigl\langle #1\bigr|}
\mathcommand[1]{\biggket}{\biggl|#1\biggr\rangle}
\mathcommand[1]{\biggbra}{\biggl\langle #1\biggr|}
\mathcommand[1]{\ket}{\left| #1 \right\rangle}  %a Ket
\mathcommand[1]{\lket}{\bigl| #1 \bigr)}  %a Liouville Ket
\mathcommand[1]{\bra}{\left\langle #1 \right|}  %a Bra
\mathcommand[1]{\lbra}{\bigl( #1 \bigr|}  %a Bra
\newcommand{\ketbra}[2]{\left| #1 \right\rangle\!\!\left\langle #2
\right|} %an outer product
\newcommand{\braket}[2]{\left\langle #1 |#2\!\right\rangle} %an inner product
\newcommand{\bigbraket}[2]{\bigl\langle #1 \bigl| #2 \bigr\rangle} %an inner product
\newcommand{\biggbraket}[2]{\biggl\langle #1 \biggl| #2 \biggr\rangle} %an inner product
\newcommand{\bigketbra}[2]{\bigl| #1 \bigr\rangle\!\bigl\langle #2
\bigr|} %an outer product
\newcommand{\lbraket}[2]{\bigl( #1 \bigl| #2 \bigr)} %an inner product
\newcommand{\lketbra}[2]{\bigl| #1 \bigr)\!\!\bigl( #2
\bigr|} %an outer product
\newcommand{\sizedlbraket}[2]{\left.\left( #1 \left| #2 \right)\right.\right.} %an inner product
\newcommand{\biglbraket}[2]{\biggl(#1\biggl|#2\biggr)}
    % This one (above) scales to the right size, but:
    % works only if bra is smaller than ket
    % If something else is needed, define \rbraket
    % These Always make big delimiters
\newcommand{\bbraket}[2]{\biggl\langle #1 \biggm| #2 \biggr\rangle}
\mathcommand[1]{\bbra}{\biggl\langle #1 \biggr|}
\mathcommand[1]{\bket}{\biggl| #1 \biggr\rangle}
\newcommand{\gsket}{\ket{\Omega}}  %Ground state
\newcommand{\gsbra}{\bra{\Omega}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Units
\mathcommand[1]{\power}{\times 10^{#1}}
\mathcommand{\tesla}{\text{~T}}
\mathcommand{\cc}{\text{~cm}^3}
%\mathcommand{\kelvin}{^\circ\text{K}}
\mathcommand{\kelvin}{\text{~K}}
\mathcommand{\percc}{\text{~cm}^{-3}}
\mathcommand{\mol}{\text{~mol}}

\mathcommand{\per}{/\!\!} %Gets rid of that hard space

\renewcommand{\deg}{\ensuremath{^\circ}}

% Energy and Power
\mathcommand{\joule}{\text{~J}}
\mathcommand{\Joule}{\text{~J}}
\mathcommand{\meV}{\text{~meV}}
\mathcommand{\eV}{\text{~eV}}
\mathcommand{\keV}{\text{~keV}}
\mathcommand{\MeV}{\text{~MeV}}
\mathcommand{\GeV}{\text{~GeV}}
\mathcommand{\uW}{\text{~}\mu\text{W}}
\mathcommand{\watts}{\text{~W}}
\mathcommand{\watt}{\watts}
\mathcommand{\volts}{\text{~V}}
% Freq
\mathcommand{\mHz}{\text{~mHz}}
\mathcommand{\Hz}{\text{~Hz}}
\mathcommand{\kHz}{\text{~kHz}}
\mathcommand{\MHz}{\text{~MHz}}
\mathcommand{\GHz}{\text{~GHz}}
\mathcommand{\THz}{\text{~THz}}
\mathcommand{\PHz}{\text{~PHz}}
% Time
\mathcommand{\yr}{\text{~yr}}
\mathcommand{\hr}{\text{~hr}}
\mathcommand{\minutes}{\text{~min}}
\mathcommand{\seconds}{\text{~sec}}
\mathcommand{\second}{\text{~sec}}
%\mathcommand{\sec}{\text{~sec}} Already defined!
\mathcommand{\ms}{\text{~ms}}
\mathcommand{\us}{\text{~}\mu\text{s}}
\mathcommand{\ns}{\text{~ns}}
\mathcommand{\ps}{\text{~ps}}
\mathcommand{\fs}{\text{~ps}}
% Length
\mathcommand{\km}{\text{~km}}
\mathcommand{\meter}{\text{~m}}
\mathcommand{\cm}{\text{~cm}}
\mathcommand{\mm}{\text{~mm}}
\mathcommand{\um}{\text{~}\mu\text{m}}
\mathcommand{\nm}{\text{~nm}}
\mathcommand{\picom}{\text{~pm}}
\mathcommand{\fm}{\text{~fm}}
\mathcommand{\angstr}{\text{~\AA}}
% Mass
\mathcommand{\gram}{\text{~g}}
\mathcommand{\kg}{\text{~kg}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% Constants
\mathcommand{\mub}{\ts{\mu}{B}}  % Bohr Magneton
\mathcommand{\kb}{\ts{k}{B}}     % Boltzmann's constant
\mathcommand{\ef}{\ts{E}{F}}     % The Fermi Energy

